CONDAQA: A Contrastive Reading Comprehension Dataset for Reasoning about Negation

The full power of human language-based communication cannot be realized without negation. All human languages have some form of negation. Despite this, negation remains a challenging phenomenon for current natural language understanding systems. To facilitate the future development of models that can process negation effectively, we present CONDAQA, the first English reading comprehension dataset which requires reasoning about the implications of negated statements in paragraphs. We collect paragraphs with diverse negation cues, then have crowdworkers ask questions about the implications of the negated statement in the passage. We also have workers make three kinds of edits to the passage -- paraphrasing the negated statement, changing the scope of the negation, and reversing the negation -- resulting in clusters of question-answer pairs that are difficult for models to answer with spurious shortcuts. CONDAQA features 14,182 question-answer pairs with over 200 unique negation cues and is challenging for current state-of-the-art models. The best performing model on CONDAQA (UnifiedQA-v2-3b) achieves only 42% on our consistency metric, well below human performance which is 81%. We release our dataset, along with fully-finetuned, few-shot, and zero-shot evaluations, to facilitate the development of future NLP methods that work on negated language.

==> figures/edit_type_model_perf.tex <==
\begin{figure}[tb]

    \includegraphics[width=\columnwidth]{figures/model_analysis/edit_types.png}

  \caption{Model accuracy based on passage type.}
 \label{ref:edittype-modelperf}
\end{figure}

==> figures/edittype_analysis.tex <==

\begin{table}[!h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc} \toprule
\textbf{Model}              & \textbf{Original} & \textbf{Paraphrase} & \textbf{Scope} & \textbf{Affirmative} \\ \midrule
UnifiedQA-V2-3B    & 75.53 & 74.23 & 69.42 & 71.43   \\
UnifiedQA-V2-Large & 68.35 & 68.13 & 63.25 & 67.22      \\
 \textsc{GPT-3}   &  57.67 & 59.79 & 51.32 & 43.91              \\
  \textsc{\faMagic InstructGPT} & 67.99 & 70.63 & 53.37 & 51.84             \\
\bottomrule        
\end{tabular}
}
\caption{Accuracy of \textsc{UnifiedQA-V2}, \textsc{GPT-3}, and \textsc{\faMagic Instruct-GPT} stratified by the type of passage.}
\label{tab:accuracy_wrt_edit_type}
\end{table}



==> figures/negation_cue_model_perf.tex <==
\begin{figure}[tb]

    \includegraphics[width=\columnwidth]{figures/model_analysis/negation_cue.png}

  \caption{Model performance on ten most frequent negation cues.}
 \label{ref:negcue-modelperf}
\end{figure}

==> tables/analysis/contrastive_train.tex <==
\begin{table}[]
\begin{tabular}{p{0.4\columnwidth} p{0.2\columnwidth} p{0.2\columnwidth}} \toprule
                         & Original test instances & All test instances \\\midrule
UnifiedQA-small-original & 50.76                   & 48.75              \\ 
UnifiedQA-base-original  & 58.28                   & 54.16              \\
UnifiedQA-large-original & 66.26                   & 62.10              \\
UnifiedQA-small          & 48.57                   & 49.03              \\
UnifiedQA-base           & 59.06                   & 56.58              \\
UnifiedQA-large          & 67.98                   & 66.15             \\ \bottomrule
\end{tabular}
\caption{Training on contrastive data vs the original dataset}
\end{table}

==> tables/question_reasoning_types_partial_new.tex <==
\begin{table*}[!tb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.025\textwidth}p{0.975\textwidth}}
\toprule
%\textbf{Reasoning Type}
%& \textbf{Example}\\
\multirow{8}{*}{\rotatebox{90}{\emph{Social Norms} (10\%)}}       & \textbf{Passage:} \textcolor{blue}{On October 8, 1883, the US patent office ruled that Edison's patent was based on the work of William E. Sawyer and was, therefore, \textbf{invalid} .} Litigation continued for nearly six years. In 1885, Latimer switched camps and started working with Edison. \textbf{Question:} From the information given in the passage, would you say that coincidence is the most charitable explanation for what was essentially the same innovation, in much the same way that Newton and Leibniz seemingly discovered calculus independently, without knowing of the other's progress?  \textbf{Answer:} YES  \\
& \textbf{Explanation:} Plagarism is frowned upon in society, more so than accidentally reaching the same conclusions as someone else.      \\
\midrule
\multirow{8}{*}{\rotatebox{90}{\emph{Psychology} (9\%)}}      &    \textbf{Passage:} [...] Disraeli later romanticised his origins, claiming his father's family was of grand Iberian and Venetian descent; in fact Isaac's family was of no great distinction [...] \textcolor{blue}{ Historians differ on Disraeli's motives for rewriting his family history: [...] Sarah Bradford believes ``his  \textbf{dislike}  of the commonplace would not allow him to accept the facts of his birth as being as middle-class and undramatic as they really were''.} \textbf{Question:} Would Disraeli have been flattered by a biography that explored his middle class upbringing, according to Bradford? \textbf{Answer:} NO   \\
& \textbf{Explanation}: A person such as Disraeli who wants to project a grandiose image of themselves is likely to be unhappy when people discuss mundane aspects about his upbringing.   \\ \midrule
\multirow{6}{*}{\rotatebox{90}{\emph{Cause \& Effect}  (7\%)}}         &     
\textbf{Passage:} Oil produced from palm fruit is called `red palm oil' or just `palm oil'... \textcolor{blue}{ In its \textbf{unprocessed}  state, red palm oil has an intense deep red color because of its abundant carotene content.} [...] \\
        &   \textbf{Question:} Would a consumer who was primarily interested in the eye-health benefits of carotenes and lycopene want to shop for palm oils by their color, rather than listening to marketing slogans such as ``extra virgin'' or ``minimally processed''? \textbf{Answer:} YES \\
        & \textbf{Explanation:} A high carotene content causes a deep red color, so a person searching for things with high carotene content can look at their color.  \\ \bottomrule    
\end{tabular}
}
\caption{Examples of questions that target the implications of negated statements in \datasetname, and reasoning steps to correctly answer the questions.  Negated statements are in \textcolor{blue}{blue}.  Categories inspired by \newcite{lobue-yates-2011-types}.}
\label{ref:qreasoning_types_partial}
\end{table*}
